Simultaneous determination of CKM angle $\gamma$ and charm mixing parameters

A combination of measurements sensitive to the $CP$ violation angle $\gamma$ of the Cabibbo-Kobayashi-Maskawa unitarity triangle and to the charm mixing parameters that describe oscillations between $D^0$ and $\bar{D}^0$ mesons is performed. Results from the charm and beauty sectors, based on data collected with the LHCb detector at CERN's Large Hadron Collider, are combined for the first time. This method provides an improvement on the precision of the charm mixing parameter $y$ by a factor of two with respect to the current world average. The charm mixing parameters are determined to be $x = (0.400^{\,+0.052}_{\,-0.053})\%$ and $y = (0.630^{\,+0.033}_{\,-0.030})\%$. The angle $\gamma$ is found to be $\gamma = (65.4^{\,+3.8}_{\,-4.2})^\circ$ and is the most precise determination from a single experiment.

==> corr_matrix_g_dh_charm.tex <==
\begin{tabular}{lrrrrrrrrrrr}
\toprule
{} &      \g &    \rdk &    \ddk &   \rdpi &   \ddpi &  \rDkpi &  \dDkpi &     \xD &     \yD &   \qopD &   \phiD \\
\midrule
\g     &  1.000 & -0.573 & -0.169 &  0.003 &  0.055 & -0.020 &  0.295 & -0.236 &  0.022 &  0.029 &  0.891 \\
\rdk   & -0.573 &  1.000 &  0.236 &  0.614 & -0.029 &  0.007 & -0.161 &  0.442 & -0.055 &  0.020 & -0.510 \\
\ddk   & -0.169 &  0.236 &  1.000 &  0.229 & -0.016 & -0.004 &  0.048 &  0.113 &  0.628 &      - & -0.180 \\
\rdpi  &  0.003 &  0.614 &  0.229 &  1.000 &      - &      - & -0.003 &  0.490 & -0.051 & -0.002 &  0.003 \\
\ddpi  &  0.055 & -0.029 & -0.016 &      - &  1.000 &  0.554 &  0.015 & -0.010 & -0.004 &  0.083 &  0.040 \\
\rDkpi & -0.020 &  0.007 & -0.004 &      - &  0.554 &  1.000 & -0.070 &  0.003 & -0.005 & -0.129 & -0.018 \\
\dDkpi &  0.295 & -0.161 &  0.048 & -0.003 &  0.015 & -0.070 &  1.000 & -0.079 &  0.084 &  0.283 & -0.096 \\
\xD    & -0.236 &  0.442 &  0.113 &  0.490 & -0.010 &  0.003 & -0.079 &  1.000 & -0.048 &  0.011 & -0.206 \\
\yD    &  0.022 & -0.055 &  0.629 & -0.051 & -0.004 & -0.005 &  0.084 & -0.048 &  1.000 & -0.005 & -0.004 \\
\qopD  &  0.029 &  0.020 &      - & -0.002 &  0.083 & -0.129 &  0.283 &  0.011 & -0.005 &  1.000 &  0.013 \\
\phiD  &  0.891 & -0.510 & -0.180 &  0.003 &  0.040 & -0.018 & -0.096 & -0.206 & -0.004 &  0.013 &  1.000 \\
\bottomrule
\end{tabular}


==> decay-def.tex <==
%
% Definition of particles.
%
\renewcommand{\Kz}     {\texorpdfstring{\ensuremath{K^0}}{K0}\xspace}

\newcommand{\hp} {\texorpdfstring{\ensuremath{h^{+}}}{h+}\xspace}
\newcommand{\hm} {\texorpdfstring{\ensuremath{h^{-}}}{h-}\xspace}
\newcommand{\hpm} {\texorpdfstring{\ensuremath{h^{\pm}}}{h-}\xspace}
\newcommand{\hmp} {\texorpdfstring{\ensuremath{h^{\mp}}}{h-}\xspace}
%
% Definition of decays.
%

%% newer style
\newcommand{\bdk}   {\texorpdfstring{\ensuremath{\Bpm\to D\Kpm}}{B -> DK}\xspace}

% Bd, Bs
\newcommand{\BDh}     {\texorpdfstring{\ensuremath{B\to Dh}}			{B -> Dh}\xspace}
\newcommand{\BDK}     {\texorpdfstring{\ensuremath{B\to DK}}			{B -> DK}\xspace}
\newcommand{\BDpi}    {\texorpdfstring{\ensuremath{B\to D\pi}}			{B -> Dpi}\xspace}

% Bu
\newcommand{\BuDpi}   {\texorpdfstring{\ensuremath{\Bu\to D \pip}}		{B+ -> Dpi+}\xspace}
\newcommand{\BuDK}    {\texorpdfstring{\ensuremath{\Bu\to D \Kp}}		{B+ -> DK+}\xspace}
\newcommand{\BuDstK}  {\texorpdfstring{\ensuremath{\Bu\to D^* \Kp}}		{B+ -> DstK+}\xspace}
\newcommand{\BuDstpi}  {\texorpdfstring{\ensuremath{\Bu\to D^* \pip}}		{B+ -> Dstpi+}\xspace}
\newcommand{\BuDsth}  {\texorpdfstring{\ensuremath{\Bu\to D^* \hp}}		{B+ -> Dsth+}\xspace}
\newcommand{\BuDKst}  {\texorpdfstring{\ensuremath{\Bu\to D K^{*+}}}		{B+ -> DstKst+}\xspace}
\newcommand{\BuDh}    {\texorpdfstring{\ensuremath{\Bu\to D h^+}}		{B+ -> Dh+}\xspace}
\newcommand{\BmDzpi}  {\texorpdfstring{\ensuremath{\Bm\to \Dz\pim}}		{B- -> D0pi-}\xspace}
\newcommand{\BmDzK}   {\texorpdfstring{\ensuremath{\Bm\to \Dz\Km}}		{B- -> D0K-}\xspace}
\newcommand{\BmDzh}   {\texorpdfstring{\ensuremath{\Bm\to \Dz h^-}}		{B- -> D0h-}\xspace}
\newcommand{\BmDzbpi} {\texorpdfstring{\ensuremath{\Bm\to \Dzb\pim}}		{B- -> D0bar pi-}\xspace}
\newcommand{\BmDzbK}  {\texorpdfstring{\ensuremath{\Bm\to \Dzb\Km}}		{B- -> D0bar K-}\xspace}
\newcommand{\BmDzbh}  {\texorpdfstring{\ensuremath{\Bm\to \Dzb h^-}}		{B- -> D0bar h-}\xspace}
\newcommand{\BpDzh}   {\texorpdfstring{\ensuremath{\Bp\to \Dz h^+}}		{B+ -> D0h+}\xspace}
\newcommand{\BpDzbh}  {\texorpdfstring{\ensuremath{\Bp\to \Dzb h^+}}		{B+ -> D0barh+\xspace}}
\newcommand{\BpmDh}   {\texorpdfstring{\ensuremath{\Bpm\to D h^\pm}}		{B+- -> Dh+-}\xspace}
\newcommand{\BpmDpi}  {\texorpdfstring{\ensuremath{\Bpm\to D \pi^\pm}}		{B+- -> Dpi+-}\xspace}
\newcommand{\BpmDK}   {\texorpdfstring{\ensuremath{\Bpm\to D K^\pm}}		{B+- -> DK+-}\xspace}
\newcommand{\BuDKpipi}{\texorpdfstring{\ensuremath{\Bu\to D \Kp\pip\pim}}		{B+ -> DK+pi+pi-}\xspace}
\newcommand{\BuDhpipi}{\texorpdfstring{\ensuremath{\Bu\to D h^+\pi\pi}}		{B+ -> Dh+pi+pi-}\xspace}

% Bd
\newcommand{\BdDpi}   {\texorpdfstring{\decay{\Bz}{\Dm \pip}}			{}}
\newcommand{\BdDpipm}   {\texorpdfstring{\decay{\Bz}{\Dmp \pipm}}		{}}
\newcommand{\BdDK}    {\texorpdfstring{\decay{\Bz}{\Dm \Kp}}			{}}
\newcommand{\BdDsp}   {\texorpdfstring{\decay{\Bz}{\Dsm \pip}}			{}}
\newcommand{\BdDspi}  {\texorpdfstring{\decay{\Bz}{\D_s \pi}}			{}}
\newcommand{\BdDsK}   {\texorpdfstring{\decay{\Bz}{\Dsm \Kp}}			{}}
\newcommand{\BdDsh}   {\texorpdfstring{\decay{\Bz}{\D_s^\mp h^\pm}}	{}}
\newcommand{\BdDsKst} {\texorpdfstring{\decay{\Bz}{\Dsm K^{*+}}}		{}}
\newcommand{\BdDzKst} {\texorpdfstring{\decay{\Bz}{\Dz K^{*0}}}		{}}
\newcommand{\BdDzKpi} {\texorpdfstring{\decay{\Bz}{\Dz K\pi}}		{}}
\newcommand{\BdDKstz} {\texorpdfstring{\decay{\Bz}{D K^{*0}}}		{}}
\newcommand{\BdDsstK} {\texorpdfstring{\decay{\Bz}{\Dssm\Kp}}			{}}
\newcommand{\BdDstpi} {\texorpdfstring{\decay{\Bz}{\Dstarm \pip}}		{}}
\newcommand{\BdDstK}  {\texorpdfstring{\decay{\Bz}{\Dstarm \Kp}}		{}}
\newcommand{\BdDrho}  {\texorpdfstring{\decay{\Bz}{\Dm \rho^{+}}}		{}}
\newcommand{\BdDsstpi}{\texorpdfstring{\decay{\Bz}{\Dstarm_s \pi}}		{}}
\newcommand{\BdDKst}  {\texorpdfstring{\decay{\Bd}{\Dm K^{*+}}}		{}}
\newcommand{\BdDKpi}  {\texorpdfstring{\decay{\Bd}{\D\Kp\pim}} {}}
\newcommand{\BdDzKstz}{\texorpdfstring{\ensuremath{\Bd\to D K^{*0}}}		{B0 -> DK*0}\xspace}
\newcommand{\BdDzbKstz}{\texorpdfstring{\ensuremath{\Bd\to\Dzb K^{*0}}}		{B0 -> DbarK*0}\xspace}
\newcommand{\BzDzKstz}{\BdDzKstz}
\newcommand{\BzDzbKstz}{\BdDzbKstz}
\newcommand{\BzDKstz}{\BdDzKstz}

% Bs
\newcommand{\BsDspi}	{\texorpdfstring{\ensuremath{\Bs\to\Dsm \pip}}		{Bs -> Dspi}\xspace}
\newcommand{\BsDsK}	{\texorpdfstring{\ensuremath{\Bs\to D_s^\mp K^\pm}}	{Bs -> DsK}\xspace}
\newcommand{\BsDsKpipi} {\texorpdfstring{\ensuremath{\Bs\to D_s^\mp K^\pm \pi^\pm \pi^\mp}} {Bs -> DsKpipi}\xspace}
\newcommand{\BsDsh}	{\texorpdfstring{\ensuremath{\Bs\to D_s^\mp h^\pm}}	{Bs -> Dsh}\xspace}
\newcommand{\BsDsmKp}	{\texorpdfstring{\ensuremath{\Bs\to D_s^- K^+}}		{Bs -> Ds-K+}\xspace}
\newcommand{\BsDspKm}	{\texorpdfstring{\ensuremath{\Bs\to D_s^+ K^-}}		{Bs -> Ds+K-}\xspace}
\newcommand{\BsDsstpi} {\decay{\Bs}{\Dsspm\pimp}}
\newcommand{\BsDsstK}  {\decay{\Bs}{\Dsspm\Kmp}}
\newcommand{\BsDstarp} {\decay{\Bs}{\Dssm \pip}}
\newcommand{\BsDstarK} {\decay{\Bs}{\Dssm \Kp}}
\newcommand{\BsDrho}   {\decay{\Bs}{\Dsm \rho^{+}}}
\newcommand{\BsDsrho}{\BsDrho}
\newcommand{\BsDsKst}   {\decay{\Bs}{\Dsm K^{*+}}}
\newcommand{\BsDstrho}   {\decay{\Bs}{\Dssm \rho^{+}}}
\newcommand{\BsDsstrho}{\BsDstrho}
\newcommand{\BsDsstKst} {\decay{\Bs}{\Dssm K^{*+}}}
\newcommand{\BsDppp}   {\decay{\Bs}{\Dsm \pip \pipi}}

% Lb
\newcommand{\LbLcK}    {\decay{\Lb}{\Lc \Km}}
\newcommand{\LbLcpi}    {\texorpdfstring{\decay{\Lb}{\Lc \pim}}{}}
\newcommand{\LbDsp}    {\texorpdfstring{\decay{\Lb}{\Dsm p}}{}}
\newcommand{\LbDsstp}    {\decay{\Lb}{\Dssm p}}

% Lc
\newcommand{\Lcpi}    {\texorpdfstring{\Lc \pim}{}}
\newcommand{\LcpKpi}    {\decay{\Lc}{p K \pi}}

% Ds
\newcommand{\DsKKpi}   {\decay{\Ds}{\Kp\Km\pip}}
\newcommand{\DspmKKpi}   {\decay{\Dspm}{\Kpm\Kmp\pipm}}
\newcommand{\Dspipipi} {\decay{\Ds}{\pip\pim\pip}}
\newcommand{\DsKpipi}  {\decay{\Ds}{\Kp\pim\pip}}
\newcommand{\Dshhh}    {\decay{\Ds}{\hp\hm\pip}}
\newcommand{\Dspmhhh}    {\decay{\Dspm}{\hpm\hmp\pipm}}

% D
% Guideline: if the D charge is given, e.g. Dz for a neutral one, the charges are displayed
% in LaTeX.
\newcommand{\DKpipi}   {\decay{\Dp}{\Km\pip\pip}}
\newcommand{\DKpipipm}   {\decay{\Dpm}{\Kmp\pipm\pipm}}
\newcommand{\DKpipipi} {\texorpdfstring{\ensuremath{D\to K^{\pm}\pi^{\mp}\pip\pim}}{D -> K3pi}\xspace}
\newcommand{\DKppp}    {\DKpipipi}
\newcommand{\DKpipiz}  {\texorpdfstring{\ensuremath{D\to K\pi\piz}}{D -> K2pi}\xspace}
\newcommand{\DKpp}     {\DKpipiz}
\newcommand{\DKpi}     {\texorpdfstring{\ensuremath{D\to K^+\pi^-}}{D -> Kpi}\xspace}
\newcommand{\DKSKpi}   {\texorpdfstring{\ensuremath{D\to \KS K^\pm\pi^\mp}}{D -> KSKpi}\xspace}
\newcommand{\DzKSKpi}  {\texorpdfstring{\ensuremath{\Dz\to \KS K^\pm\pi^\mp}}{D -> KSKpi}\xspace}
\newcommand{\DzKpi}    {\texorpdfstring{\ensuremath{\Dz\to K^\pm\pi^\mp}}{D0 -> Kpi}\xspace}
\newcommand{\DKpipm}    {\texorpdfstring{\ensuremath{\D\to K^\pm\pi^\mp}}{D -> Kpi}\xspace}
\newcommand{\DzBarKpiFav} {\texorpdfstring{\ensuremath{\Dzb\to\Kp\pim}}{D0 -> K-pi+}\xspace}
\newcommand{\DzKpiFav} {\texorpdfstring{\ensuremath{\Dz\to\Km\pip}}{D0 -> K-pi+}\xspace}
\newcommand{\DzKpiSup} {\texorpdfstring{\ensuremath{\Dz\to\pim\Kp}}{D0 -> pi-K+}\xspace}
\newcommand{\DzBarKpiSup} {\texorpdfstring{\ensuremath{\Dzb\to\pip\Km}}{D0 -> pi-K+}\xspace}
\newcommand{\DzKpipipi}{\texorpdfstring{\ensuremath{\Dz\to K^\pm\pi^\mp\pi^+\pi^-}}{D -> K3pi}\xspace}
\newcommand{\Dzhpipipi}{\texorpdfstring{\ensuremath{\Dz\to h^\pm\pi^\mp\pi^+\pi^-}}{D -> h3pi}\xspace}
\newcommand{\Dzhhpiz}  {\texorpdfstring{\ensuremath{\Dz \to h^\pm h^\mp \piz}}{D -> hhpi0}\xspace}
\newcommand{\DzKpipiz} {\texorpdfstring{\ensuremath{\Dz \to K^\pm\pi^\mp \piz}}{D -> Kpipi0}\xspace}
\newcommand{\DzKpipizFav} {\texorpdfstring{\ensuremath{\Dz \to \Km\pip\piz}}{D -> Kpipi0}\xspace}
\newcommand{\DzKpipizSup} {\texorpdfstring{\ensuremath{\Dz \to \Kp\pim\piz}}{D -> Kpipi0}\xspace}
\newcommand{\DzKpppFav}{\texorpdfstring{\ensuremath{\Dz\to\Km\pip\pim\pip}}{D -> K3pi (fav)}\xspace}
\newcommand{\DzKpppSup}{\texorpdfstring{\ensuremath{\Dz\to\pim\Kp\pim\pip}}{D -> K3pi (sup)}\xspace}
\newcommand{\DzKppp}{\DzKpipipi}
\newcommand{\DzKpipipiFav}{\DzKpppFav}
\newcommand{\DzKpipipiSup}{\DzKpppSup}
\newcommand{\DzKpp}{\DzKpipiz}
\newcommand{\DzKppFav}{\DzKpipizFav}
\newcommand{\DzKppSup}{\DzKpipizSup}
\newcommand{\Dhh}      {\texorpdfstring{\ensuremath{D\to h^+h^-}}{D -> hh}\xspace}
\newcommand{\Dhhh}     {\texorpdfstring{\ensuremath{D\to hhhh}}{D -> hhhh}\xspace}
\newcommand{\Dhpipipi} {\texorpdfstring{\ensuremath{D\to h^+\pi^-\pi^+\pi^-}}{D -> hpipipi}\xspace}
\newcommand{\Dpipipipi} {\texorpdfstring{\ensuremath{D\to \pi^+\pi^-\pi^+\pi^-}}{D -> hpipipi}\xspace}
\newcommand{\Dzpipipipi} {\texorpdfstring{\ensuremath{D\to \pi\pi\pi\pi}}{D -> hpipipi}\xspace}
\newcommand{\Dhhpiz}   {\texorpdfstring{\ensuremath{D\to h^+h^-\piz}}{D -> hhpi0}\xspace}
\newcommand{\Dzhh}     {\texorpdfstring{\ensuremath{\Dz\to h^+h^-}}{D -> hh}\xspace}
\newcommand{\DzKK}     {\texorpdfstring{\ensuremath{\Dz\to K^+K^-}}{D -> KK}\xspace}
\newcommand{\DKK}     {\texorpdfstring{\ensuremath{D\to K^+K^-}}{D -> KK}\xspace}
\newcommand{\Dzpipi}   {\texorpdfstring{\ensuremath{\Dz\to\pi^+\pi^-}}{D -> pipi}\xspace}
\newcommand{\Dpipi}   {\texorpdfstring{\ensuremath{D\to\pi^+\pi^-}}{D -> pipi}\xspace}
\newcommand{\DzKShh}   {\texorpdfstring{\ensuremath{\Dz\to\KS h^+h^-}}{D0 -> KShh}\xspace}
\newcommand{\DKSpipi}  {\texorpdfstring{\ensuremath{D\to\KS\pi^+\pi^-}}{D -> KSpipi}\xspace}
\newcommand{\DKSKK}    {\texorpdfstring{\ensuremath{D\to\KS K^+K^-}}{D -> KSKK}\xspace}
\newcommand{\DKShh}    {\texorpdfstring{\ensuremath{D\to\KS h^+h^-}}{D -> KShh}\xspace}
\newcommand{\Dzpipipiz} {\texorpdfstring{\ensuremath{\Dz\to\pi^+\pi^-\piz}}{D -> pipipi0}\xspace}
\newcommand{\DzKKpiz}   {\texorpdfstring{\ensuremath{\Dz\to K^+ K^-\piz}}{D -> KKpi0}\xspace}
\newcommand{\Dpipipiz} {\texorpdfstring{\ensuremath{D\to\pi^+\pi^-\piz}}{D -> pipipi0}\xspace}
\newcommand{\DKKpiz}   {\texorpdfstring{\ensuremath{D\to K^+ K^-\piz}}{D -> KKpi0}\xspace}

% K decays
\newcommand{\KstKSpi}{\texorpdfstring{\ensuremath{\Kstarp\to\KS\pip}}{K*+ -> KSpi+}\xspace}

% B final states
\newcommand{\DzK}      {\texorpdfstring{\ensuremath{DK^\pm}}{DK}\xspace}
\newcommand{\Dzpi}     {\texorpdfstring{\ensuremath{D\pi^\pm}}{Dpi}\xspace}
\newcommand{\DsK}      {\texorpdfstring{\ensuremath{D_s K}}{DsK}\xspace}
\newcommand{\Dspi}     {\ensuremath{D_s \pi}\xspace}
\newcommand{\DsKp}     {\ensuremath{\Dsm\Kp}\xspace}
\newcommand{\DsKm}     {\ensuremath{\Ds\Km}\xspace}
\newcommand{\Dpi}      {\texorpdfstring{\ensuremath{D\pi}}{Dpi}\xspace}

% D final states
\newcommand{\KK}   		{\texorpdfstring{\ensuremath{\Kp\Km}}{K+K-}\xspace}
\newcommand{\pipi}   		{\texorpdfstring{\ensuremath{\pip\pim}}{pi+pi-}\xspace}
\newcommand{\pipipipi}   		{\texorpdfstring{\ensuremath{\pip\pim\pip\pim}}{pi+pi-pi+pi-}\xspace}
\newcommand{\Kpi}   		{\texorpdfstring{\ensuremath{\Kpm\pimp}}{K+/-pi-/+}\xspace}
\newcommand{\Kpipipi}  		{\texorpdfstring{\ensuremath{\Kpm\pimp\pip\pim}}{Kpipipi}\xspace}
\newcommand{\KSKpi}  		{\texorpdfstring{\ensuremath{\KS\Kpm\pimp}}{KSKpi}\xspace}
\newcommand{\KSpipi}  		{\texorpdfstring{\ensuremath{\KS\pip\pim}}{KSpipi}\xspace}
\newcommand{\KSKK}  		{\texorpdfstring{\ensuremath{\KS\Kp\Km}}{KSKK}\xspace}
\newcommand{\KKpiz}  		{\texorpdfstring{\ensuremath{\Kp\Km\piz}}{KKpiz}\xspace}
\newcommand{\Kpipiz}  		{\texorpdfstring{\ensuremath{\Kpm\pimp\piz}}{Kpipiz}\xspace}
\newcommand{\pipipiz}  		{\texorpdfstring{\ensuremath{\pip\pim\piz}}{pipipiz}\xspace}

% to match output of first
\newcommand{\bdh}{\BDh}
\newcommand{\bdsth}{\BuDsth}
\newcommand{\bdkst}{\BuDKst}
\newcommand{\bdkstz}{\BdDKstz}
\newcommand{\bdhpp}{\BuDhpipi}
\newcommand{\bsdsk}{\BsDsK}
\newcommand{\bsdskpp}{\BsDsKpipi}

==> parameter-def.tex <==
%
% Definition of gamma related parameters.
%

%
% PARAMETERS
%

% phases (already in lhcb-symbols-def.tex)
\renewcommand{\g}{\texorpdfstring{\ensuremath{\gamma}}{gamma}\xspace}
\renewcommand{\phis}{\texorpdfstring{\ensuremath{\phi_s}}{phis}\xspace}

% generic symbols for hadronic parameters
\newcommand{\rb}   {\texorpdfstring{\ensuremath{r_B}}{rB}\xspace}
\newcommand{\db}   {\texorpdfstring{\ensuremath{\delta_B}}{dB}\xspace}
\newcommand{\kb}   {\texorpdfstring{\ensuremath{\kappa_B}}{kB}\xspace}
\newcommand{\rbsq} {\texorpdfstring{\ensuremath{r_B^2}}{rB2}\xspace}
\newcommand{\rd}   {\texorpdfstring{\ensuremath{r_D}}{rD}\xspace}
\newcommand{\dd}   {\texorpdfstring{\ensuremath{\delta_D}}{dD}\xspace}
\newcommand{\kd}   {\texorpdfstring{\ensuremath{\kappa_D}}{kD}\xspace}
\newcommand{\rdsq} {\texorpdfstring{\ensuremath{r_D^2}}{rD2}\xspace}
\newcommand{\Fp}   {\texorpdfstring{\ensuremath{F^{+}}}{Fp}\xspace}

% B+ -> DK+/B+ -> Dpi+
\newcommand{\Rcab} {\texorpdfstring{\ensuremath{R_{\rm Cab.}}}{Rcab}\xspace}

% B+ -> D0K+
\newcommand{\rbdk} {\texorpdfstring{\ensuremath{r_{\Bpm}^{D\Kpm}}}{rBDK}\xspace}
\newcommand{\dbdk} {\texorpdfstring{\ensuremath{\delta_{\Bpm}^{D\Kpm}}}{dBDK}\xspace}

% B+ -> D0pi+
\newcommand{\rbdpi} {\texorpdfstring{\ensuremath{r_{\Bpm}^{D\pipm}}}{rBDpi}\xspace}
\newcommand{\dbdpi} {\texorpdfstring{\ensuremath{\delta_{\Bpm}^{D\pipm}}}{dBDpi}\xspace}

% B+ -> D*0K+
\newcommand{\rbdstk}{\texorpdfstring{\ensuremath{r_{\Bpm}^{D^{*}\Kpm}}}{rBD*K}\xspace}
\newcommand{\dbdstk}{\texorpdfstring{\ensuremath{\delta_{\Bpm}^{D^{*}\Kpm}}}{dBD*K}\xspace}
\newcommand{\kbdstk}{\texorpdfstring{\ensuremath{\kappa_{\Bpm}^{D^{*}\Kpm}}}{kBD*K}\xspace}

% B+ -> D*0pi+
\newcommand{\rbdstpi}{\texorpdfstring{\ensuremath{r_{\Bpm}^{D^{*}\pipm}}}{rBD*pi}\xspace}
\newcommand{\dbdstpi}{\texorpdfstring{\ensuremath{\delta_{\Bpm}^{D^{*}\pipm}}}{dBD*pi}\xspace}
\newcommand{\kbdstpi}{\texorpdfstring{\ensuremath{\kappa_{\Bpm}^{D^{*}\pipm}}}{kBD*pi}\xspace}

% B+ -> D0K*+
\newcommand{\rbdkst}{\texorpdfstring{\ensuremath{r_{\Bpm}^{D\Kstarpm}}}{rBDK*}\xspace}
\newcommand{\dbdkst}{\texorpdfstring{\ensuremath{\delta_{\Bpm}^{D\Kstarpm}}}{dBDK*}\xspace}
\newcommand{\kbdkst}{\texorpdfstring{\ensuremath{\kappa_{\Bpm}^{D\Kstarpm}}}{kBDK*}\xspace}

% B0 -> D0K*0
\newcommand{\rbdkstz}{\texorpdfstring{\ensuremath{r_{\Bd}^{D\Kstarz}}}{rBDK*0}\xspace}
\newcommand{\dbdkstz}{\texorpdfstring{\ensuremath{\delta_{\Bd}^{D\Kstarz}}}{dBDK*0}\xspace}
\newcommand{\kbdkstz}{\texorpdfstring{\ensuremath{\kappa_{\Bd}^{D\Kstarz}}}{kBDK*0}\xspace}

% B+ -> D0K+pipi
\newcommand{\rbdkpipi}{\texorpdfstring{\ensuremath{r_{\Bd}^{D\Kpm\pip\pim}}}{rBDKpipi}\xspace}
\newcommand{\dbdkpipi}{\texorpdfstring{\ensuremath{\delta_{\Bd}^{D\Kpm\pip\pim}}}{dBDKpipi}\xspace}
\newcommand{\kbdkpipi}{\texorpdfstring{\ensuremath{\kappa_{\Bd}^{D\Kpm\pip\pim}}}{kBDKpipi}\xspace}

% B+ -> D0pi+pipi
\newcommand{\rbdpipipi}{\texorpdfstring{\ensuremath{r_{\Bd}^{D\pipm\pip\pim}}}{rBDpipipi}\xspace}
\newcommand{\dbdpipipi}{\texorpdfstring{\ensuremath{\delta_{\Bd}^{D\pipm\pip\pim}}}{dBDpipipi}\xspace}
\newcommand{\kbdpipipi}{\texorpdfstring{\ensuremath{\kappa_{\Bd}^{D\pipm\pip\pim}}}{kBDpipipi}\xspace}

% B0 -> D-pi+
\newcommand{\lbdmpip}{\texorpdfstring{\ensuremath{\lambda_\Bd^{\Dmp\pipm}}\xspace}{l_Dpi}}
\newcommand{\rbdmpip}{\texorpdfstring{\ensuremath{r_\Bd^{\Dmp\pipm}}\xspace}{r_Dpi}}
\newcommand{\dbdmpip}{\texorpdfstring{\ensuremath{\delta_\Bd^{\Dmp\pipm}}\xspace}{delta_Dpi}}

% Bs -> DsK
\newcommand{\lbsdsk}{\texorpdfstring{\ensuremath{\lambda_\Bs^{\Dsmp\Kpm}}\xspace}{l_DsK}}
\newcommand{\rbsdsk}{\texorpdfstring{\ensuremath{R_\Bs^{\Dsmp\Kpm}}\xspace}{r_DsK}}
\newcommand{\dbsdsk}{\texorpdfstring{\ensuremath{\delta_B^{\Dsmp\Kpm}}\xspace}{delta_DsK}}

% Bs -> DsKpipi
\newcommand{\lbsdskpipi}{\texorpdfstring{\ensuremath{\lambda_\Bs^{\Dsmp\Kpm\pip\pim}}\xspace}{l_DsKpipi}}
\newcommand{\rbsdskpipi}{\texorpdfstring{\ensuremath{R_\Bs^{\Dsmp\Kpm\pip\pim}}}{rDsKpipi}\xspace}
\newcommand{\dbsdskpipi}{\texorpdfstring{\ensuremath{\delta_\Bs^{\Dsmp\Kpm\pip\pim}}}{dDsKpipi}\xspace}
\newcommand{\kbsdskpipi}{\texorpdfstring{\ensuremath{\kappa_\Bs^{\Dsmp\Kpm\pip\pim}}}{kDsKpipi}\xspace}

% Charm
\newcommand{\xd}{\texorpdfstring{\ensuremath{x_D}\xspace}{xD}}
\newcommand{\yd}{\texorpdfstring{\ensuremath{y_D}\xspace}{yD}}
\newcommand{\xcp}{\texorpdfstring{\ensuremath{x_{\CP}}\xspace}{xCP}}
\renewcommand{\ycp}{\texorpdfstring{\ensuremath{y_{\CP}}\xspace}{yCP}}
\newcommand{\Deltax}{\texorpdfstring{\ensuremath{\Delta x}\xspace}{Dx}}
\newcommand{\Deltay}{\texorpdfstring{\ensuremath{\Delta y}\xspace}{Dy}}
\newcommand{\qopd}{\texorpdfstring{\ensuremath{|q/p|_D}\xspace}{qopD}}
\renewcommand{\phid}{\texorpdfstring{\ensuremath{\phi_D}\xspace}{phiD}}
\newcommand{\xD}{\xd}
\newcommand{\yD}{\yd}
\newcommand{\qopD}{\qopd}
\newcommand{\phiD}{\phid}

% generic symbols
\newcommand{\rbh}  {\texorpdfstring{\ensuremath{r_B^h}}{rBh}\xspace}
\newcommand{\rbhsq}{\texorpdfstring{\ensuremath{(r_B^{h})^2}}{rBh2}\xspace}
\newcommand{\dbh}  {\ensuremath{\delta_B^h}\xspace}
\newcommand{\kbh}  {\texorpdfstring{\ensuremath{\kappa_B^h}}{kBh}\xspace}
\newcommand{\dD}{\texorpdfstring{\ensuremath{\delta_{D}}}{dD}\xspace}
\newcommand{\kD}{\texorpdfstring{\ensuremath{\kappa_{D}}}{kD}\xspace}

% B+ -> DK+
\newcommand{\rbk}  {\texorpdfstring{\ensuremath{r_B^{DK}}}{rBDK}\xspace}
\newcommand{\rbksq}{\texorpdfstring{\ensuremath{(r_B^{DK})^2}}{rBDK2}\xspace}
\newcommand{\dbk}  {\ensuremath{\delta_B^{DK}}\xspace}

% B+ -> Dpi+
\newcommand{\rbpi}  {\texorpdfstring{\ensuremath{r_B^{D\pi}}}{rBDpi}\xspace}
\newcommand{\rbpisq}{\texorpdfstring{\ensuremath{(r_B^{D\pi})^2}}{rBDpi2}\xspace}
\newcommand{\dbpi}  {\ensuremath{\delta_B^{D\pi}}\xspace}

% B+ -> Dhpipi
\newcommand{\rbDkpp}{\ensuremath{r_B^{DK\pi\pi}}\xspace}
\newcommand{\rbDkppsq}{\ensuremath{(\rbDkpp)^2}\xspace}
\newcommand{\dbDkpp}{\ensuremath{\delta_B^{DK\pi\pi}}\xspace}
\newcommand{\kbDkpp}{\ensuremath{\kappa_B^{DK\pi\pi}}\xspace}
\newcommand{\rbDppp}{\ensuremath{r_B^{D\pi\pi\pi}}\xspace}
\newcommand{\rbDpppsq}{\ensuremath{(\rbDppp)^2}\xspace}
\newcommand{\dbDppp}{\ensuremath{\delta_B^{D\pi\pi\pi}}\xspace}
\newcommand{\kbDppp}{\ensuremath{\kappa_B^{D\pi\pi\pi}}\xspace}

% B+ -> D0*K+
\newcommand{\rbDstKp}{\ensuremath{r_B^{D^{*}K^{+}}}\xspace}
\newcommand{\dbDstKp}{\ensuremath{\delta_B^{D^{*}K^{+}}}\xspace}
\newcommand{\kbDstKp}{\ensuremath{\kappa_B^{D^{*}K^{+}}}\xspace}
\newcommand{\rbsqDstKp}{\texorpdfstring{\ensuremath{(r_B^{D^{*}K^{+}})^2}}{rBDstK2}\xspace}

% B+ -> D0K*+
\newcommand{\rbDKstp}{\ensuremath{r_B^{DK^{*+}}}\xspace}
\newcommand{\dbDKstp}{\ensuremath{\delta_B^{DK^{*+}}}\xspace}
\newcommand{\kbDKstp}{\ensuremath{\kappa_B^{DK^{*+}}}\xspace}
\newcommand{\rbsqDKstp}{\texorpdfstring{\ensuremath{(r_B^{DK^{*+}})^2}}{rBDKst2}\xspace}

% B0 -> D0K*0
\newcommand{\rbDKpi}{\ensuremath{r_B^{DK\pi}}\xspace}
\newcommand{\rbDKstz}{\ensuremath{r_B^{DK^{*0}}}\xspace}
\newcommand{\rbbarDKstz}{\ensuremath{\bar{r}_B^{DK^{*0}}}\xspace}
\newcommand{\rbDKstzsq}{\ensuremath{\left(r_B^{DK^{*0}}\right)^2}\xspace}
\newcommand{\rbbarDKstzsq}{\ensuremath{\left(\bar{r}_B^{DK^{*0}}\right)^2}\xspace}
\newcommand{\dbDKstz}{\ensuremath{\delta_B^{DK^{*0}}}\xspace}
\newcommand{\dbDKpi}{\ensuremath{\delta_B^{DK\pi}}\xspace}
\newcommand{\dbbarDKstz}{\ensuremath{\bar{\delta}_B^{DK^{*0}}}\xspace}
\newcommand{\kbDKstz}{\ensuremath{\kappa_B^{DK^{*0}}}\xspace}
\newcommand{\RbDKstz}{\ensuremath{\bar{R}_{B}^{DK^{*0}}}\xspace}
\newcommand{\DbDKstz}{\ensuremath{\bar{\Delta}_{B}^{DK^{*0}}}\xspace}
\newcommand{\RBDKstz}{\ensuremath{\bar{R}_{B}^{DK^{*0}}}\xspace}
\newcommand{\DBDKstz}{\ensuremath{\bar{\Delta}_{B}^{DK^{*0}}}\xspace}

% B0 -> Dpi
\newcommand{\rbdmpi}{\texorpdfstring{\ensuremath{r_B^{D^\mp\pi^\pm}}\xspace}{r_Dpi}}
\newcommand{\rbdmpisq}{\texorpdfstring{\ensuremath{(r_B^{D^\mp\pi^\pm})^2}}{rDpi^2}\xspace}
\newcommand{\dbdmpi}{\texorpdfstring{\ensuremath{\delta_B^{D^\mp\pi^\pm}}\xspace}{delta_Dpi}}

% Bs -> DsK
\newcommand{\rdsk}{\texorpdfstring{\ensuremath{r_B^{D_s^\mp K^\pm}}}{rDsK}\xspace}
\newcommand{\rdsksq}{\texorpdfstring{\ensuremath{(r_B^{D_s^\mp K^\pm})^2}}{rDsK^2}\xspace}
%\newcommand{\ddsk}{\texorpdfstring{\ensuremath{\delta_B^{D_s^\mp K^\pm}}}{dDsK}\xspace}
\renewcommand{\phis}{\texorpdfstring{\ensuremath{\phi_s}}{phis}\xspace}

% Bs -> DsKpipi
\newcommand{\rdskpipi}{\texorpdfstring{\ensuremath{r_B^{D_s^\mp K^\pm\pimp\pipm}}}{rDsKpipi}\xspace}
\newcommand{\rdskpipisq}{\texorpdfstring{\ensuremath{(r_B^{D_s^\mp K^\pm\pimp\pipm})^2}}{rDsKpipi^2}\xspace}
\newcommand{\kdskpipi}{\texorpdfstring{\ensuremath{\kappa_B^{D_s^\mp K^\pm\pimp\pipm}}}{kDsKpipi}\xspace}

% D -> f_flv
\newcommand{\rdFlv}  {\ensuremath{r_{f}}\xspace}
\newcommand{\rdFlvsq}{\ensuremath{r_{f}^2}\xspace}
\newcommand{\ddFlv}  {\ensuremath{\delta_{f}}\xspace}
\newcommand{\kdFlv}  {\ensuremath{\kappa_{f}}\xspace}

% D -> Kpi
\newcommand{\rdKpi}  {\ensuremath{r_D^{K\pi}}\xspace}
\newcommand{\rdKpisq}{\ensuremath{(r_D^{K\pi})^2}\xspace}
\newcommand{\ddKpi}  {\ensuremath{\delta_D^{K\pi}}\xspace}
\newcommand{\ddKpicos}  {\ensuremath{\cos\delta_D^{K\pi}}\xspace}
\newcommand{\ddKpisin}  {\ensuremath{\sin\delta_D^{K\pi}}\xspace}
\newcommand{\RdKpi}  {\ensuremath{R_D^{K\pi}}\xspace}

% D -> Kpipiz
\newcommand{\rdKpp}{\ensuremath{r_{D}^{K2\pi}}\xspace}
\newcommand{\rdKppsq}{\ensuremath{(r_{D}^{K2\pi})^{2}}\xspace}
\newcommand{\ddKpp}{\ensuremath{\delta_{D}^{K2\pi}}\xspace}
\newcommand{\kdKpp}{\ensuremath{\kappa_{D}^{K2\pi}}\xspace}
\newcommand{\Fppp}{\ensuremath{F_{\pi\pi\piz}}\xspace}
\newcommand{\FKKp}{\ensuremath{F_{KK\piz}}\xspace}
\newcommand{\kdppp}{\ensuremath{\kappa_{\pi\pi\piz}}\xspace}
\newcommand{\kdkkp}{\ensuremath{\kappa_{KK\piz}}\xspace}
\newcommand{\Aprod}{\ensuremath{A_{B}^{\rm{prod}}}\xspace}

% D -> KSKpi
\newcommand{\rdKskpi}{\ensuremath{r_D^{K_SK\pi}}\xspace}
\newcommand{\rdKskpisq}{\ensuremath{(r_D^{K_SK\pi})^2}\xspace}
\newcommand{\ddKskpi}{\ensuremath{\delta_D^{K_SK\pi}}\xspace}
\newcommand{\kdKskpi}{\ensuremath{\kappa_D^{K_SK\pi}}\xspace}
\newcommand{\RdKskpi}{\ensuremath{R_D^{K_SK\pi}}\xspace}

\newcommand{\rdKstK}{\ensuremath{r_D^{K^*K}}\xspace}
\newcommand{\rdKstKsq}{\ensuremath{(r_D^{K^*K})^2}\xspace}
\newcommand{\ddKstK}{\ensuremath{\delta_D^{K^*K}}\xspace}
\newcommand{\kdKstK}{\ensuremath{\kappa_D^{K^*K}}\xspace}
\newcommand{\RdKstK}{\ensuremath{R_D^{K^*K}}\xspace}

% D -> hpipipi
\newcommand{\rdKppp}{\texorpdfstring{\ensuremath{r_D^{K3\pi}}}{rD(K3pi)}\xspace}
\newcommand{\rdKpppsq}{\ensuremath{(r_D^{K3\pi})^2}\xspace}
\newcommand{\ddKppp}{\ensuremath{\delta_D^{K3\pi}}\xspace}
\newcommand{\kdKppp}{\ensuremath{\kappa_D^{K3\pi}}\xspace}
\newcommand{\Fpppp}{\ensuremath{F_{4\pi}}\xspace}
\newcommand{\kdpppp}{\ensuremath{\kappa_{4\pi}}\xspace}
\newcommand{\RdKpipipi}  {\ensuremath{R_D^{K3\pi}}\xspace}

% charm
\newcommand{\dAcp}{\texorpdfstring{\ensuremath{\Delta a^{\rm dir}_{\CP}}\xspace}{DeltaAdir}}
\newcommand{\DAcpKK}  {\texorpdfstring{\ensuremath{A_{\CP}^{\rm dir}(KK)}\xspace}{AcpDir(KK)}}
\newcommand{\DAcpPipi}{\texorpdfstring{\ensuremath{A_{\CP}^{\rm dir}(\pi\pi)}\xspace}{AcpDir(pipi}}
\newcommand{\DAcpKpi}{\texorpdfstring{\ensuremath{A_{\CP}^{\rm dir}(K\pi)}\xspace}{AcpDir(Kpi}}
\newcommand{\DAcphh}  {\texorpdfstring{\ensuremath{A_{\CP}^{\rm dir}}\xspace}{Acp(D->fCP)}}
\newcommand{\DAcphhalt} {\texorpdfstring{\ensuremath{A_{\CP}^{\rm dir}(hh)}\xspace}{AcpDir(hh)}}
\newcommand{\brKpppFav}{\texorpdfstring{\ensuremath{\mathcal{B}(\DzKpppFav)}}{B(D0->Kpipipi)}\xspace}
\newcommand{\brKpppSup}{\texorpdfstring{\ensuremath{\mathcal{B}(\DzKpppSup)}}{B(D0->piKpipi)}\xspace}


%
% OBSERVABLES
%

% charm CPV
\newcommand{\dAcpobs}{\texorpdfstring{\ensuremath{a^{\rm dir}_{\CP,\rm obs}}\xspace}{deltaAcpObs}}
\newcommand{\DAcpKKobs}{\texorpdfstring{\ensuremath{A_{\CP,\rm obs}^{KK}}\xspace}{DAcpKKObs}}
\newcommand{\DAcpPipiobs}{\texorpdfstring{\ensuremath{A_{\CP,\rm obs}^{\pi\pi}}\xspace}{DAcpPipiObs}}

% D->hh
\newcommand{\AGamma}{\texorpdfstring{\ensuremath{A_\Gamma}\xspace}{AGamma}}

% D->K3pi
\newcommand{\RM}{\texorpdfstring{\ensuremath{R_M}\xspace}{RM}}
\newcommand{\RMhalf}{\texorpdfstring{\ensuremath{R_M/2}\xspace}{RMhalf}}

% charm mixing
\newcommand{\dRD}{\texorpdfstring{\ensuremath{R_D}\xspace}{RD}}
\newcommand{\xdsq}{\texorpdfstring{\ensuremath{x_D^2}\xspace}{xD'2}}
\newcommand{\ydsq}{\texorpdfstring{\ensuremath{y_D^2}\xspace}{yD'2}}
\newcommand{\xdprimesq}{\texorpdfstring{\ensuremath{x_D^{\prime2}}\xspace}{xD'2}}
\newcommand{\xdprime}{\texorpdfstring{\ensuremath{x'_D}\xspace}{xD'}}
\newcommand{\ydprime}{\texorpdfstring{\ensuremath{y'_D}\xspace}{yD'}}
\newcommand{\ydprimekpipipi}{\texorpdfstring{\ensuremath{y'^{K3\pi}_D}\xspace}{yD'}}
\newcommand{\dRDp}{\texorpdfstring{\ensuremath{R_D^+}\xspace}{RDp}}
\newcommand{\dRDm}{\texorpdfstring{\ensuremath{R_D^-}\xspace}{RDm}}
\newcommand{\xdprimesqp}{\texorpdfstring{\ensuremath{(x_D^{\prime +})^2}\xspace}{xD'2p}}
\newcommand{\xdprimesqm}{\texorpdfstring{\ensuremath{(x_D^{\prime -})^2}\xspace}{xD'2m}}
\newcommand{\ydprimep}{\texorpdfstring{\ensuremath{y^{\prime +}_D}\xspace}{yD'p}}
\newcommand{\ydprimem}{\texorpdfstring{\ensuremath{y^{\prime -}_D}\xspace}{yD'm}}
\newcommand{\xdprimep}{\texorpdfstring{\ensuremath{x^{\prime +}_D}\xspace}{xD'p}}
\newcommand{\xdprimem}{\texorpdfstring{\ensuremath{x^{\prime -}_D}\xspace}{xD'm}}

% D->Kpi auxiliary input
\newcommand{\rdKpiObs}{\ensuremath{r_{K\pi,\rm obs}}\xspace}
\newcommand{\ddKpiObs}{\ensuremath{\delta_{K\pi, \rm obs}}\xspace}

% D->K3pi auxiliary input
\newcommand{\RWSKpipipi}{\ensuremath{R_{WS}(\DKpipipi)}\xspace}
\newcommand{\RWSKpipiz}{\ensuremath{R_{WS}(\DKpipiz)}\xspace}

% DK GGSZ
\newcommand{\xm} {\ensuremath{x_-}\xspace}
\newcommand{\ym} {\ensuremath{y_-}\xspace}
\newcommand{\xpm}{\ensuremath{x_\pm}\xspace}
\newcommand{\xp} {\ensuremath{x_+}\xspace}
\newcommand{\yp} {\ensuremath{y_+}\xspace}
\newcommand{\ypm}{\ensuremath{y_\pm}\xspace}

%DK+Dpi GGSZ
\newcommand{\xmdk} {\ensuremath{x_-^{DK}}\xspace}
\newcommand{\ymdk} {\ensuremath{y_-^{DK}}\xspace}
\newcommand{\xpmdk}{\ensuremath{x_\pm^{DK}}\xspace}
\newcommand{\xpdk} {\ensuremath{x_+^{DK}}\xspace}
\newcommand{\ypdk} {\ensuremath{y_+^{DK}}\xspace}
\newcommand{\ypmdk}{\ensuremath{y_\pm^{DK}}\xspace}
\newcommand{\xdpi} {\ensuremath{x_\xi^{D\pi}}\xspace}
\newcommand{\ydpi} {\ensuremath{y_\xi^{D\pi}}\xspace}

% DK* BDKpi
\newcommand{\xmdkst} {\ensuremath{x_-^{D\Kstarz}}\xspace}
\newcommand{\ymdkst} {\ensuremath{y_-^{D\Kstarz}}\xspace}
\newcommand{\xpmdkst}{\ensuremath{x_\pm^{D\Kstarz}}\xspace}
\newcommand{\xpdkst} {\ensuremath{x_+^{D\Kstarz}}\xspace}
\newcommand{\ypdkst} {\ensuremath{y_+^{D\Kstarz}}\xspace}
\newcommand{\ypmdkst}{\ensuremath{y_\pm^{D\Kstarz}}\xspace}
\newcommand{\xmdkpi} {\ensuremath{x_-^{DK\pi}}\xspace}
\newcommand{\ymdkpi} {\ensuremath{y_-^{DK\pi}}\xspace}
\newcommand{\xpmdkpi}{\ensuremath{x_\pm^{DK\pi}}\xspace}
\newcommand{\xpdkpi} {\ensuremath{x_+^{DK\pi}}\xspace}
\newcommand{\ypdkpi} {\ensuremath{y_+^{DK\pi}}\xspace}
\newcommand{\ypmdkpi}{\ensuremath{y_\pm^{DK\pi}}\xspace}

% GLW
\newcommand{\Acp}{\ensuremath{A_{\CP}}\xspace}
\newcommand{\Acpp}{\ensuremath{A_{\CP\!+}}\xspace}
\newcommand{\Acpm}{\ensuremath{A_{\CP\!-}}\xspace}
\newcommand{\Acppm}{\ensuremath{A_{\CP\!\pm}}\xspace}
\newcommand{\Rcp}{\ensuremath{R_{\CP}}\xspace}
\newcommand{\Rcpp}{\ensuremath{R_{\CP\!+}}\xspace}
\newcommand{\Rcpm}{\ensuremath{R_{\CP\!-}}\xspace}
\newcommand{\Rcppm}{\ensuremath{R_{\CP\!\pm}}\xspace}

% ADS
\newcommand{\Rp}{\ensuremath{R_+}\xspace}
\newcommand{\Rm}{\ensuremath{R_-}\xspace}
\newcommand{\Rpm}{\ensuremath{R_\pm}\xspace}
\newcommand{\Rads}{\ensuremath{R_{\rm ADS}}\xspace}
\newcommand{\Aads}{\ensuremath{A_{\rm ADS}}\xspace}

% D*K, D->hh GLW
\newcommand{\AcpDkDg}{\ensuremath{A_{\CP}^{D\gamma K}}\xspace}
\newcommand{\AcpDkDp}{\ensuremath{A_{\CP}^{D\piz K}}\xspace}
\newcommand{\AcpDpiDg}{\ensuremath{A_{\CP}^{D\gamma\pi}}\xspace}
\newcommand{\AcpDpiDp}{\ensuremath{A_{\CP}^{D\piz\pi}}\xspace}
\newcommand{\RcpDkDg}{\ensuremath{R_{\CP}^{D\gamma}}\xspace}
\newcommand{\RcpDkDp}{\ensuremath{R_{\CP}^{D\piz}}\xspace}
\newcommand{\AfavDkDg}{\ensuremath{A_{\rm fav}^{D\gamma, K\pi}}\xspace}
\newcommand{\AfavDkDp}{\ensuremath{A_{\rm fav}^{D\piz, K\pi}}\xspace}
\newcommand{\RpDkKpiDg}{\ensuremath{R_+^{D\gamma K,K\pi}}\xspace}
\newcommand{\RmDkKpiDg}{\ensuremath{R_-^{D\gamma K,K\pi}}\xspace}
\newcommand{\RpDpiKpiDg}{\ensuremath{R_+^{D\gamma \pi,K\pi}}\xspace}
\newcommand{\RmDpiKpiDg}{\ensuremath{R_-^{D\gamma \pi,K\pi}}\xspace}
\newcommand{\RpDkKpiDp}{\ensuremath{R_+^{D\piz K,K\pi}}\xspace}
\newcommand{\RmDkKpiDp}{\ensuremath{R_-^{D\piz K,K\pi}}\xspace}
\newcommand{\RpDpiKpiDp}{\ensuremath{R_+^{D\piz \pi,K\pi}}\xspace}
\newcommand{\RmDpiKpiDp}{\ensuremath{R_-^{D\piz \pi,K\pi}}\xspace}
\newcommand{\AfavDkKpiDg}{\ensuremath{A_{\rm fav}^{D\gamma K, K\pi}}\xspace}
\newcommand{\AfavDkKpiDp}{\ensuremath{A_{\rm fav}^{D\piz K, K\pi}}\xspace}
\newcommand{\AfavDpiKpiDg}{\ensuremath{A_{\rm fav}^{D\gamma\pi, K\pi}}\xspace}
\newcommand{\AfavDpiKpiDp}{\ensuremath{A_{\rm fav}^{D\piz\pi, K\pi}}\xspace}
\newcommand{\RkpKpiDg}{\ensuremath{R_{K/\pi}^{D\gamma, K\pi}}\xspace}
\newcommand{\RkphhDg}{\ensuremath{R_{K/\pi}^{D\gamma, hh}}\xspace}
\newcommand{\RkpKpiDp}{\ensuremath{R_{K/\pi}^{D\piz, K\pi}}\xspace}
\newcommand{\RkphhDp}{\ensuremath{R_{K/\pi}^{D\piz, hh}}\xspace}

% D->hh GLW/ADS
\newcommand{\AcpDkKK}{\ensuremath{A_{\CP}^{KK}}\xspace}
\newcommand{\AcpDkPipi}{\ensuremath{A_{\CP}^{\pi\pi}}\xspace}
\newcommand{\AcpDk}{\ensuremath{A_{\CP}^{DK}}\xspace}
\newcommand{\AcpDpiKK}{\ensuremath{A_{\CP}^{D\pi, KK}}\xspace}
\newcommand{\AcpDpiPipi}{\ensuremath{A_{\CP}^{D\pi, \pi\pi}}\xspace}
\newcommand{\AcpDpi}{\ensuremath{A_{\CP}^{D\pi}}\xspace}
\newcommand{\AfavDkKpi}{\ensuremath{A_{\rm fav}^{K\pi}}\xspace}
\newcommand{\AfavDpiKpi}{\ensuremath{A_{\rm fav}^{D\pi, K\pi}}\xspace}
\newcommand{\RpDkKpi}{\ensuremath{R_+^{DK,K\pi}}\xspace}
\newcommand{\RmDkKpi}{\ensuremath{R_-^{DK,K\pi}}\xspace}
\newcommand{\RpDpiKpi}{\ensuremath{R_+^{D\pi,K\pi}}\xspace}
\newcommand{\RmDpiKpi}{\ensuremath{R_-^{D\pi,K\pi}}\xspace}
\newcommand{\RkpKpi}{\ensuremath{R_{K/\pi}^{K\pi}}\xspace}
\newcommand{\RkpKK}{\ensuremath{R_{K/\pi}^{KK}}\xspace}
\newcommand{\RkpPipi}{\ensuremath{R_{K/\pi}^{\pi\pi}}\xspace}
\newcommand{\Rkphh}{\ensuremath{R_{K/\pi}^{hh}}\xspace}
\newcommand{\RCPKK}{\ensuremath{R_{CP}^{KK}}\xspace}
\newcommand{\RCPPiPi}{\ensuremath{R_{CP}^{\pi\pi}}\xspace}
\newcommand{\RadsDK}{\ensuremath{R_{\rm{ADS}}^{\pi K}}\xspace}
\newcommand{\RadsDPi}{\ensuremath{R_{\rm{ADS}(\pi)}^{K\pi}}\xspace}
\newcommand{\AadsDK}{\ensuremath{A_{\rm{ADS}}^{\pi K}}\xspace}
\newcommand{\AadsDPi}{\ensuremath{A_{\rm{ADS}(\pi)}^{K\pi}}\xspace}

% D->K3pi ADS
\newcommand{\AfavDkKppp}{\ensuremath{A_{\rm fav}^{K3\pi}}\xspace}
\newcommand{\AcpDKpppp}{\ensuremath{A_{\CP}^{4\pi}}\xspace}
\newcommand{\AcpDPipppp}{\ensuremath{A_{\CP}^{D\pi,4\pi}}\xspace}
\newcommand{\AfavDpiKppp}{\ensuremath{A_{\rm fav}^{D\pi, K3\pi}}\xspace}
\newcommand{\RpDkKppp}{\ensuremath{R_+^{DK,K3\pi}}\xspace}
\newcommand{\RmDkKppp}{\ensuremath{R_-^{DK,K3\pi}}\xspace}
\newcommand{\RpDpiKppp}{\ensuremath{R_+^{D\pi,K3\pi}}\xspace}
\newcommand{\RmDpiKppp}{\ensuremath{R_-^{D\pi,K3\pi}}\xspace}
\newcommand{\RkpKppp}{\ensuremath{R_{K/\pi}^{K3\pi}}\xspace}
\newcommand{\Rkppppp}{\ensuremath{R_{K/\pi}^{4\pi}}\xspace}
\newcommand{\RCPKppp}{\ensuremath{R_{CP}^{K3\pi}}\xspace}
\newcommand{\RCPpppp}{\ensuremath{R_{CP}^{4\pi}}\xspace}
\newcommand{\RadsDKKppp}{\ensuremath{R_{\rm{ADS}}^{K3\pi}}\xspace}
\newcommand{\RadsDPiKppp}{\ensuremath{R_{\rm{ADS}(\pi)}^{K3\pi}}\xspace}
\newcommand{\AadsDKKppp}{\ensuremath{A_{\rm{ADS}}^{K3\pi}}\xspace}
\newcommand{\AadsDPiKppp}{\ensuremath{A_{\rm{ADS}(\pi)}^{K3\pi}}\xspace}

% D->hhpiz GLW/ADS
\newcommand{\AcpDkKKPiz}{\ensuremath{A_{\CP}^{KK\piz}}\xspace}
\newcommand{\AcpDkPiPiPiz}{\ensuremath{A_{\CP}^{\pi\pi\piz}}\xspace}
\newcommand{\AcpDpiKKPiz}{\ensuremath{A_{\CP}^{D\pi, KK\piz}}\xspace}
\newcommand{\AcpDpiPiPiPiz}{\ensuremath{A_{\CP}^{D\pi, \pi\pi\piz}}\xspace}
\newcommand{\AfavDkKPiPiz}{\ensuremath{A_{\rm fav}^{K\pi\piz}}\xspace}
\newcommand{\AfavDPiKPiPiz}{\ensuremath{A_{\rm fav}^{D\pi, K\pi\piz}}\xspace}
\newcommand{\RCPKKPiz}{\ensuremath{R_{CP}^{KK\piz}}\xspace}
\newcommand{\RCPPiPiPiz}{\ensuremath{R_{CP}^{\pi\pi\piz}}\xspace}
\newcommand{\RadsDKkpp}{\ensuremath{R_{\rm{ADS}}^{K\pi\piz}}\xspace}
\newcommand{\RadsDPikpp}{\ensuremath{R_{\rm{ADS}(\pi)}^{K\pi\piz}}\xspace}
\newcommand{\AadsDKkpp}{\ensuremath{A_{\rm{ADS}}^{K\pi\piz}}\xspace}
\newcommand{\AadsDPikpp}{\ensuremath{A_{\rm{ADS}(\pi)}^{K\pi\piz}}\xspace}

% D->KSKpi GLS
\newcommand{\RfavsupDpiKskpi}{\ensuremath{R_{D\pi,\,\rm fav/sup}^{K_SK\pi}}\xspace}
\newcommand{\RfavDkDpiKskpi}{\ensuremath{R_{K/\pi,\,\rm fav}^{K_SK\pi}}\xspace}
\newcommand{\RsupDkDpiKskpi}{\ensuremath{R_{K/\pi,\,\rm sup}^{K_SK\pi}}\xspace}
\newcommand{\AfavDkKskpi}{\ensuremath{A_{\rm fav}^{K_SK\pi}}\xspace}
\newcommand{\AsupDkKskpi}{\ensuremath{A_{\rm sup}^{K_SK\pi}}\xspace}
\newcommand{\AfavDpiKskpi}{\ensuremath{A_{\rm fav}^{D\pi,\,K_SK\pi}}\xspace}
\newcommand{\AsupDpiKskpi}{\ensuremath{A_{\rm sup}^{D\pi,\,K_SK\pi}}\xspace}
\newcommand{\RfavsupDkKskpi}{\ensuremath{R^{K_SK\pi}}\xspace}

% B0->DK*0, D->hh, hhhh GLW/ADS
\newcommand{\AcpDkstKK}{\ensuremath{A_{\CP}^{D\Kstarz,\,KK}}\xspace}
\newcommand{\AfavDkstKpi}{\ensuremath{A_{\rm fav}^{D\Kstarz,\,K\pi}}\xspace}
\newcommand{\RcpDkstKK}{\ensuremath{R_{\CP}^{D\Kstarz,\,KK}}\xspace}
\newcommand{\AcpDkstPipi}{\ensuremath{A_{\CP}^{D\Kstarz,\,\pi\pi}}\xspace}
\newcommand{\RcpDkstPipi}{\ensuremath{R_{\CP}^{D\Kstarz,\,\pi\pi}}\xspace}
\newcommand{\RpDkstKpi}{\ensuremath{R_+^{D\Kstarz,\,K\pi}}\xspace}
\newcommand{\RmDkstKpi}{\ensuremath{R_-^{D\Kstarz,\,K\pi}}\xspace}
\newcommand{\RcpDksthh}{\ensuremath{R_{\CP}^{D\Kstarz,\,hh}}\xspace}
\newcommand{\AfavDkstKpipipi}{\ensuremath{A_{\rm fav}^{D\Kstarz,\,K3\pi}}\xspace}
\newcommand{\AcpDkstPipipipi}{\ensuremath{A_{\CP}^{D\Kstarz,\,4\pi}}\xspace}
\newcommand{\RcpDkstPipipipi}{\ensuremath{R_{\CP}^{D\Kstarz,\,4\pi}}\xspace}
\newcommand{\RpDkstKpipipi}{\ensuremath{R_+^{D\Kstarz,\,K3\pi}}\xspace}
\newcommand{\RmDkstKpipipi}{\ensuremath{R_-^{D\Kstarz,\,K3\pi}}\xspace}

% B+->DK+*, D->hh GLW/ADS
\newcommand{\AcpDkstpKK}{\ensuremath{A_{\CP}^{D\Kstarp,\,KK}}\xspace}
\newcommand{\AfavDkstpKpi}{\ensuremath{A_{\rm fav}^{D\Kstarp,\,K\pi}}\xspace}
\newcommand{\RcpDkstpKK}{\ensuremath{R_{\CP}^{D\Kstarp,\,KK}}\xspace}
\newcommand{\AcpDkstpPipi}{\ensuremath{A_{\CP}^{D\Kstarp,\,\pi\pi}}\xspace}
\newcommand{\RcpDkstpPipi}{\ensuremath{R_{\CP}^{D\Kstarp,\,\pi\pi}}\xspace}
\newcommand{\RpDkstpKpi}{\ensuremath{R_+^{D\Kstarp,\,K\pi}}\xspace}
\newcommand{\RmDkstpKpi}{\ensuremath{R_-^{D\Kstarp,\,K\pi}}\xspace}
\newcommand{\RcpDkstphh}{\ensuremath{R_{\CP}^{D\Kstarp,\,hh}}\xspace}

% B+->DK+*, D->hhhh GLW/ADS
\newcommand{\AfavDkstpKpipipi}{\ensuremath{A_{\rm fav}^{D\Kstarp,\,K3\pi}}\xspace}
\newcommand{\AcpDkstpPipipipi}{\ensuremath{A_{\CP}^{D\Kstarp,\,4\pi}}\xspace}
\newcommand{\RcpDkstpPipipipi}{\ensuremath{R_{\CP}^{D\Kstarp,\,4\pi}}\xspace}
\newcommand{\RpDkstpKpipipi}{\ensuremath{R_+^{D\Kstarp,\,K3\pi}}\xspace}
\newcommand{\RmDkstpKpipipi}{\ensuremath{R_-^{D\Kstarp,\,K3\pi}}\xspace}

% B->Dhpipi, D->hh GLW/ADS
\newcommand{\RcpDkpipi}{\ensuremath{R_{\CP}^{DK\pi\pi}}\xspace}
\newcommand{\AfavDkpipiKpi}{\ensuremath{A_{\rm fav}^{DK\pi\pi,\,K\pi}}\xspace}
\newcommand{\AfavDpipipiKpi}{\ensuremath{A_{\rm fav}^{D\pi\pi\pi,\,K\pi}}\xspace}
\newcommand{\AcpDkpipiKK}{\ensuremath{A_{\CP}^{DK\pi\pi,\,KK}}\xspace}
\newcommand{\AcpDkpipiPipi}{\ensuremath{A_{\CP}^{DK\pi\pi,\,\pi\pi}}\xspace}
\newcommand{\AcpDpipipiKK}{\ensuremath{A_{\CP}^{D\pi\pi\pi,\,KK}}\xspace}
\newcommand{\AcpDpipipiPipi}{\ensuremath{A_{\CP}^{D\pi\pi\pi,\,\pi\pi}}\xspace}
\newcommand{\RpDkpipiKpi}{\ensuremath{R_+^{DK\pi\pi,\,K\pi}}\xspace}
\newcommand{\RmDkpipiKpi}{\ensuremath{R_-^{DK\pi\pi,\,K\pi}}\xspace}
\newcommand{\RpDpipipiKpi}{\ensuremath{R_+^{D\pi\pi\pi,\,K\pi}}\xspace}
\newcommand{\RmDpipipiKpi}{\ensuremath{R_-^{D\pi\pi\pi,\,K\pi}}\xspace}

% DsK
% use DsK analysis team notation
\newcommand{\Cpar}	{\ensuremath{C}\xspace}
\newcommand{\Dpar}	{\ensuremath{D_f}\xspace}
\newcommand{\Dbpar}	{\ensuremath{D_{\bar{f}}}\xspace}
\newcommand{\Spar}	{\ensuremath{S_f}\xspace}
\newcommand{\Sbpar}	{\ensuremath{S_{\bar{f}}}\xspace}

% DsKpipi
\newcommand{\CparDsKpipi}	{\ensuremath{C^{\Ds K\pi\pi}}\xspace}
\newcommand{\DparDsKpipi}	{\ensuremath{D^{\Ds K\pi\pi}_f}\xspace}
\newcommand{\DbparDsKpipi}	{\ensuremath{D^{\Ds K\pi\pi}_{\bar{f}}}\xspace}
\newcommand{\SparDsKpipi}	{\ensuremath{S^{\Ds K\pi\pi}_f}\xspace}
\newcommand{\SbparDsKpipi}	{\ensuremath{S^{\Ds K\pi\pi}_{\bar{f}}}\xspace}

% Dpi
\newcommand{\Spardpi}  {\ensuremath{S^{D\pi}_f}\xspace}
\newcommand{\Sbpardpi}  {\ensuremath{S^{D\pi}_{\bar{f}}}\xspace}

% from Bs->DsK ANA
\def\fdsk{\ensuremath{f}\xspace}
\def\fbdsk{\ensuremath{\bar{f}}\xspace}
\def\lbdsk{\ensuremath{\overline{\lambda}_{\fbdsk}}\xspace}
\def\Afdsk{\ensuremath{A_{\fdsk}}\xspace}
\def\Afbdsk{\ensuremath{A_{\fbdsk}}\xspace}
\def\Abfdsk{\ensuremath{\overline{A}_{\fdsk}}\xspace}
\def\Abfbdsk{\ensuremath{\overline{A}_{\fbdsk}}\xspace}
\def\Cfdsk{\ensuremath{C_{\fdsk}}\xspace}
\def\Cfbdsk{\ensuremath{C_{\fbdsk}}\xspace}
\def\Dfdsk{\ensuremath{D_{\fdsk}}\xspace}
\def\Dfbdsk{\ensuremath{D_{\fbdsk}}\xspace}
\def\Sfdsk{\ensuremath{S_{\fdsk}}\xspace}
\def\Sfbdsk{\ensuremath{S_{\fbdsk}}\xspace}

\def\normlamsq{\ensuremath{|\ldsk|^2}\xspace}
\def\normlambarsq{|\bar{\lambda}_{\fbdsk}|^{2}}
\def\deltag{\frac{\Delta \Gamma_{s} \, t}{2}}
\def\dMst{\Delta m_{s} \, t}
\def\poverq{\Big|\frac{p}{q}\Big|^{2}}
\def\qoverp{\Big|\frac{q}{p}\Big|^{2}}
\def\weak{\gamma - 2\beta_s}

% to help our results tables if we don't have them already
% these are the variables as defined in the code with the
% underscores removed and 0's replaced with z's
\newcommand{\rdk}{\rbdk}
\newcommand{\ddk}{\dbdk}
\newcommand{\rdpi}{\rbdpi}
\newcommand{\ddpi}{\dbdpi}
\newcommand{\rdstk}{\rbdstk}
\newcommand{\ddstk}{\dbdstk}
\newcommand{\rdstpi}{\rbdstpi}
\newcommand{\ddstpi}{\dbdstpi}
\newcommand{\rdkst}{\rbdkst}
\newcommand{\ddkst}{\dbdkst}
\newcommand{\kdkst}{\kbdkst}
\newcommand{\rdkstz}{\rbdkstz}
\newcommand{\ddkstz}{\dbdkstz}
\newcommand{\kdkstz}{\kbdkstz}
\newcommand{\rdkpipi}{\rbdkpipi}
\newcommand{\ddkpipi}{\dbdkpipi}
\newcommand{\kdkpipi}{\kbdkpipi}
\newcommand{\rdpipipi}{\rbdpipipi}
\newcommand{\ddpipipi}{\dbdpipipi}
\newcommand{\kdpipipi}{\kbdpipipi}
\newcommand{\ldsk}{\rbsdsk}
\newcommand{\ddsk}{\dbsdsk}
\newcommand{\ldskpipi}{\rbsdskpipi}
\newcommand{\ddskpipi}{\dbsdskpipi}
\newcommand{\ldmpi}{\rbdmpi}
\newcommand{\ddmpi}{\dbdmpi}
\newcommand{\rDkpi}{\rdKpi}
\newcommand{\dDkpi}{\ddKpi}
\newcommand{\rDkpipiz}{\rdKpp}
\newcommand{\dDkpipiz}{\ddKpp}
\newcommand{\kDkpipiz}{\kdKpp}
\newcommand{\rDkpipipi}{\rdKppp}
\newcommand{\dDkpipipi}{\ddKppp}
\newcommand{\kDkpipipi}{\kdKppp}
\newcommand{\rDkskpi}{\rdKskpi}
\newcommand{\dDkskpi}{\ddKskpi}
\newcommand{\kDkskpi}{\kdKskpi}
\newcommand{\Fkkpiz}{\FKKp}
\newcommand{\Fpipipiz}{\Fppp}
\newcommand{\Fpipipipi}{\Fpppp}
\newcommand{\RBRdkdpi}{\Rcab}
